Spider: A Large-Scale Human-Labeled Dataset for Complex and Cross-Domain Semantic Parsing and Text-to-SQL Task

We present Spider, a large-scale, complex and cross-domain semantic parsing and text-to-SQL dataset annotated by 11 college students. It consists of 10,181 questions and 5,693 unique complex SQL queries on 200 databases with multiple tables, covering 138 different domains. We define a new complex and cross-domain semantic parsing and text-to-SQL task where different complex SQL queries and databases appear in train and test sets. In this way, the task requires the model to generalize well to both new SQL queries and new database schemas. Spider is distinct from most of the previous semantic parsing tasks because they all use a single database and the exact same programs in the train set and the test set. We experiment with various state-of-the-art models and the best model achieves only 12.4% exact matching accuracy on a database split setting. This shows that Spider presents a strong challenge for future research. Our dataset and task are publicly available at https://yale-lily.github.io/spider

==> obsolete/annotation_projection.tex <==
As discussed in \S\ref{sec_background}, we can use the same supervised system that we train on the labeled examples in the source language to train on the projected data. We use the  Naive Bayes Support Vector Machine (NBSVM) model of \newcite{??} which is an extension of \namecite{?}.
\todo{KM: I think we should make clear this is our own modification of Manning}
\todo{MSR: I think it is good to cite to Anonymous and mention that it is an extension of Manning.}
\todo{Yes. I agree with this. I've added mention of extension}
We use this model as our supervised and projection model because it outperforms many state-of-the-art neural network systems in the supervised setting. 
\todo{KM: Tao: what do you mean "Either". Don't you mean both? How is it either?}
This models makes use of either bi-gram or tri-gram features. It uses a log-count ratio vector between the word counts in positive cases and the word counts in negative cases as weights for the n-gram feature vectors\todo{this is not clear to me how you extracted the counts}. The method uses word embedding features grouped by part-of-speech tags
\todo{KM: Clarify. Do you mean you produce a word embedding for all nouns? What do you mean grouped by part-of-speech?}
and adds sentiment and negation word indicator tokens at the end of each sentence in conjunction with the log-ratio vector.
\todo{KM: Please add an example. I think that would help explain. I don't know what you're adding.}

We include all features only when English is the source language. For other languages, we only use the word embeddings grouped by POS tags and n-gram features without appending sentiment lexicon and negation word indicator tokens at the end of sentences for each language. As mentioned in \S\ref{sec_background}, when we have multiple sources of translation for a target language, we apply majority voting to get the most frequent label as our final decision for projection.


\todo{KM: This is better than before but I Think could still use some clarification.}

==> obsolete/approach.tex <==
\label{sec_approach}
This section gives a detailed description  of the proposed transfer models.



\subsection{Annotation Projection}
\input{annotation_projection}
\subsection{Direct Transfer}
\input{direct_transfer}


==> obsolete/background.tex <==
\label{sec_background}

This section gives a description of the underlying transfer models used in our experiments.
\begin{comment}


\subsection{Supervised Sentiment Analysis}\label{sec_sup_sent}
\todo{KM: Agree this section can be removed.}
In a supervised sentiment analysis system, a set of training examples ${\cal X}=\{x_1, x_2, \cdots, x_n\}$ are given with their corresponding labels $\{l_1, l_2, \cdots, l_n\}$. Each label $l_i$ comes from the set of possible sentiment labels ${\cal L}=\{positive, negative, neutral\}$. A machine learning method learns a model ${\cal M}$ from the labeled instances ${\cal X}$. At decoding time, the sentiment analysis system uses a scoring function obtained from ${\cal M}$ and predicts the best label $l^*(x)$ for every sentence $x$: 

\[
l^*(x) = \arg\max_{l \in {\cal L}} \theta(\phi(x,l))
\]

where $\theta(x,l)$ is a function that gives the score of label $l$ for the input sentence $x$. The function $\phi(x,l)\in \mathbb{R}^d$ is a generic feature function that extracts features for sentence $x$ and label $l$. The features may include any useful information such as word n-grams, part-of-speech tags or word embeddings. 


\subsection{Data Assumption}
Throughout this paper, we will assume that we have $k$ source languages $L_1, \cdots, L_k$ and a single target language $L_{k+1}$. We assume to have the following data:

\begin{itemize}
    \item Labeled training examples ${\cal X}_i$ for $i\in \{1,\cdots,k\}$.
    \item Small translation data for all language pairs. We can also extract a cross-lingual translation dictionary $t(w, i, j)$ for which gives the most frequent translation of word $w$ in language $i$ to language $j$. The frequency of translations is automatically extracted from word alignment (e.g. Giza++~\cite{och2000giza}) run on translation data. 
    \item Part-of-speech tagger and word tokenizer for all languages. 
    \item Monolingual text for all languages. We use the Wikipedia text in this paper.
\end{itemize}


\subsection{A Baseline Approach}\label{sec_baseline}
As a baseline, we use a lexicon-based approach. We use the Sentiwordnet lexicon \cite{baccianella2010sentiwordnet}: this lexicon gives the probability of each word and sense pair for being positive or negative. Formally, we use the lexicon ${\cal S}$ that gives the probability of positive and negative sentiments as a two-dimensional vector  ${\cal S}(w,s)\in \mathbb{R}^2$ for a word $w$ and its corresponding sense $s$. Since we do not have word sense information for the target language, we use the averaged vector $\psi(w)\in \mathbb{R}^2$ over all the possible senses of each word $w$:

\[
 \psi(w)= 
\begin{cases}
   \frac{\sum_{s \in \text{senses}(w)} {\cal S}(w,s)}{|\text{senses}(w)|} & \text{if } w\in {\cal S}\\        [0, 0]         & \text{otherwise}
\end{cases}\]

 For each sentence $x$ in a target language $L_t$, we use the translation dictionary to get the corresponding English Sentiwordnet score and average them by the number of seen entries in the Sentiwordnet dictionary: 
 
\[
f(x) = \frac{\sum_{i=1}^{n} \psi(t(w_i, \text{en}, L_t))}{\sum_{i=1}^{n}\mathbb{I}(t(w_i, \text{en}, L_t)\in {\cal S})}
\]

where $\mathbb{I}$ is the identity function.

Finally we define a simple threshold to assign the label of the sentence:

\[
l(x)=
\begin{cases}
\text{positive} & f(x)[0]-f(x)[1]>\delta \\
\text{negative} & f(x)[1]-f(x)[0]>\delta \\
\text{neutral} & \text{otherwise} \\
\end{cases}
\]

where $f(x)[0]$ and $f(x)[1]$ show the positive and negative scores of sentence $x$ and $\delta$ is a predefined threshold. In this paper we use $\delta = 0.1$.
\end{comment}

\subsection{Annotation Projection}
In single-source annotation projection, we assume that we have translation data where sentences $\{s_1, s_2, \cdots, s_m\}$ from the source rich-resource language $L_s$ are translated to sentences  $\{t_1, t_2, \cdots, t_m\}$ in a low-resource language $L_t$; i.e. $s_i$ is a translation for $t_i$ for $i=1,\cdots, m$. We also assume that we have labeled training examples ${\cal X}=\{x_1, x_2, \cdots, x_n\}$ for the source language $L_s$. Thus, we first train a supervised system ${\cal M}_{sup}$ on ${\cal X}$ and afterward, use the trained system to  ${\cal M}_{sup}$ predict the labels of the source-side parallel translated text  $\{l_{s_1}, l_{s_2}, \cdots, l_{s_m}\}$. We project those labels to the target-side translation by assuming $l_{s_i} \rightarrow l_{t_i}$.  After applying projection, we use the target-side translation text $\{t_1, t_2, \cdots, t_m\}$ with the projected labels  $\{l_{t_1}, l_{t_2}, \cdots, l_{t_m}\}$ to train the target model ${\cal M}_{proj}$. The trained model ${\cal M}_{proj}$ is  the final model for analyzing sentiment in the target language.

Multi-source transfer is an extension to single-source transfer. In this setting, there is more than one source language and the translation data includes a mapping between source sentences in multiple source languages for each target sentence. In this setting,  we apply the same technique for each source language and use majority voting the get the most reliable projected label for each target sentence. Finally, a supervised system is trained on the projected data.



\subsection{Direct Transfer}
In direct transfer, we directly use the training instance $X_i$ for the source languages $L_i$ ($i=1,\cdots k$). We can have an unrestricted number of source languages. In other words, a supervised sentiment analysis system can be trained on the concatenation of $k$ labeled datasets $\cup_{i=1}^{k} {\cal X}_i$ or can be the outcome of the ensemble of $k$ single-source direct transfer methods. One benefit of direct transfer is the direct use of gold labels in code-switched data as opposed to the use of automatically transferred  labels in annotation projection. The main problem with direct transfer is that most of the common features do not generalize beyond each source language: for example lexical features in one language may not appear in other languages. To address this problem, we design a deep learning neural network model that makes use of cross-lingual word representations and translation dictionaries. More details are given in \S\ref{sec_direct}.



==> obsolete/direct_transfer.tex <==
\label{sec_direct}
This subsection explains our direct transfer model by describing the feature adaption approach and the deep learning model.


\subsubsection{Feature Adaptation}
As mentioned in \S\ref{sec_background}, the main challenge in direct transfer is the adaptation of features from the source languages to the target language. When dealing with labeled datasets in other languages, most of the words occurring in the training data do not exist in the target language vocabulary. We apply the following techniques to address this problem:

\begin{itemize}
    \item {\bf Word representation features:} We train cross-lingual word representations such that words with similar meanings in different language have similar representations. We use the method of \newcite[Figure 1]{rasooli_16} to train cross-lingual word embeddings and Brown clusters.
    \item {\bf Lexical features:}  We use the translation dictionaries $t(w, i, t)$ that are either extracted from the translation text or from manual dictionaries to translate as many words of the labeled examples ${\cal X}_i \in L_i$ to the target language words.
\todo{KM: Mohammad - do you use any lexical features other than the words themselves? Or are you referring to the word embeddings of the translated words? It's slightly unclear what you mean by lexical features. Perhaps you should define it if you're going to use it often?} 
The lexical features of the translated words can be used directly when training the target model. 

\end{itemize}

\subsubsection{Deep Learning Model}
The input to our model is a sequence of words in the sentence $x = \{x_1, x_2, \cdots, x_n\}$ where $n$ is the number of words. If any dictionary (either extracted from parallel data or a manual dictionary) is provided, the words that exist in the dictionary, will be translated to the target language. The model uses two representations for the input: a recurrent representation based on long short-term memories (LSTM) \cite{hochreiter1997long} and the other based on averaging over all inputs. A graphical depiction of underlying model is shown in Figure~\ref{fig_neural_fig}.
\todo{KM: In this section, I don't think it is clear that you use code-switched data. Unless perhaps it is in a later section? I am wondering if some examples would help.}
\todo{KM: YOu definitely need an example here. Show the code-switched data and describe how that affects the word embeddings.}

\input{neural_fig}

\paragraph{Embedding Layer}
We use the following features for every word in the sentence:

\begin{itemize}
    \item A \emph{fixed} pre-trained cross-lingual word embeddings $x_{ce} \in \mathbb{R}^{d_{ce}}$ extracted from the method of \newcite{rasooli_16}. %If a word is translated and its translation has an entry in the word embeddings dictionary, we use that as the feature; otherwise we use the original word as the input feature. 
    \item A randomly initialized word embedding $x_{e} \in \mathbb{R}^{d_{e}}$ for every word in the sentence. 
\todo{KM: I would not comment out the following sentence as it's unclear here whether you have a sentence in one language or if you have both.}
If a word has translation, we use the translation; otherwise we use the original word. 
    \item The cross-lingual word cluster embedding $x_{cc} \in \mathbb{R}^{d_{cc}}$ to represent the word cluster identity of each word. The word clusters are extracted by the method of \newcite{rasooli_16}.
\todo{KM: Again, I would include the sentence you have commented below. I have uncommented both.}
Similar to the cross-lingual embeddings; we first look at the translation and otherwise the original word. 
\todo{KM: Are you using sentiwordnet in *all* methods? I thought you were just using it in the baseline.}
    \item In the case of single transfer from English, we use the fixed two-dimensional Sentiwordnet \cite{baccianella2010sentiwordnet} score $x_{sw} \in \mathbb{R}^{2}$ that represents the likelihood of a word being positive or negative. We basically translate Sentiwordnet lexicon to the target language by using the translation dictionaries.
\end{itemize}


\paragraph{Intermediate Layer}
The input for every word $x_i$ to intermediate layers is the concatenation of the embedding layers: $f = x_{ce}[i] \circ  x_e[i] \circ x_{cc}[i]$ where $\circ$ is the concatenation operator. Thus the dimension of the input is $d_i = d_{ce}+d_{e}+d_{cc}$.\footnote{For the sake of generality, we have not included the Sentiwordnet representation $x_{sw}$ in the notation since it is only used in single-transfer from English to the target and not in the multi-source transfer experiments.} The following representations are used to represent the intermediate layer:

\begin{itemize}
    \item {\bf Recurrent layer}: We use a Bidirectional LSTM (BiLSTM) for representing the sequence of words in the sentence: a forward pass $LSTM_f(f_{[1:n]}) \in \mathbb{R}^{d_{rec} \times d_i}$ gives the final representation of the sentence by looking from left to right, and the backward pass $LSTM_b(f_{[n:1]}) \in \mathbb{R}^{d_{rec} \times d_i}$ looks from right to left. Then the output of the two LSTMs are concatenated as $r(x) \in \mathbb{R}^{2\cdot d_{rec}}$:
    \[
    r(x) = LSTM_f(f_{[1:n]}) \circ LSTM_b(f_{[n:1]})
    \]
    
    \item {\bf Average pool layer}: Since there are so many word order inconsistencies from the source to the target languages, we also use an average pool layer $p(x) \in \mathbb{R}^{d_i}$ to average all the input features. This layer is represents the bag-of-word information of the sentence without taking the sequence information into account: 
    \[
    p(x) = \frac{\sum_{i=1}^{n} f[i]}{n}
    \]
\end{itemize}


\paragraph{Output Layer}
We use a multilayer perceptron (MLP) to get the likelihood of each label: the two intermediate layers $r(x)$ and $p(x)$ are concatenated and fed to a hidden layer $H \in \mathbb{R}^{d_h \times (2\cdot d_{rec} + d_i)}$ activated by  rectified linear units (ReLU) \cite{nair2010rectified}:

\[
 H(x) = ReLU (H  (r(x) \circ p(x))
\]

Finally the hidden layer output is fed to the output softmax layer with the weight matrix $W \in \mathbb{R}^{|{\cal L}| \times d_h}$ where $|{\cal L}|$ is the number of unique sentiment labels (in our case it is 3):

\[
p(l | x) = \frac{e_l^{W  H(x)}}{\sum_{i=1}^{|{\cal L}|} e_i^{W  H(x)}}
\]

We use the sum log likelihood function function with the Adam optimizer \cite{adam_paper} to learn the model parameters.


==> obsolete/discussion.tex <==
\todo{MSR: will write this after having all results}


outlines: 1) compare single-source and multi-source, 2) compare projection and direct, 3) compare with and without dictionary (need to add its table), 4) more insights

{\bf KM: I have put in a short paragraph based on the results I see for single source. Tao indicated in his email last night that these are correct. We need to discuss what is LR. What are the data sizes for each and what makes them Low resource? I could take a guess based on the languages (e.g., I would guess that Slovenia and Bulgaria are lower resource than Spanish), but we should have a definition. That could help for discussion of results.}

\subsection{Transfer from a Single Source}

The results from single source transfer are mixed, but some trends do appear. In general, in-domain data (LDC) enables significant increases in performance for most languages. For projection, the LDC results are better than projection results using either BQ or EP in all cases except for Uyghur where perhaps the smaller parallel data caused the drop {\bf KM: numbers could help here. How much smaller was the Uyghur dataset than the others?}. For direct transfer, the LDC results are better than the projection results using either Wikipedia, BQ or EP in all cases except for Farsi. {\bf Mohammad - any idea why?}  

Looking at direct transfer in isolation, we see that the  automatically generated dictionaries produce better results than the manual Wikipedia dictionary in eight out of 14 languages when the BQ parallel data is used {\bf Mohammed - is there less parallel data in the other six languages?} and six out of nine  languages when the EP data is used. In general, where more parallel data is available, we can expect automatically generated dictionaries to do better than manual. 

In comparing project with direct transfer, the results are more mixed. With LDC data, each approach does better or equal on approximately the same number of languages. With the BQ data (a lower resource setting), annotation does better on average but that is because of some large differences in a small number of languages (sk, sl, sv, ug, and zh). {\bf What is different about these languages? MOre or less data? By the way, in the table there is room to spell out the language. Why not do that?} With the EP data, results are split, with direct transfer doing better on four out of nine languages, projection better on four, and in one case, equivalent performance. {\bf I think it would be worth doing statistical significance tests on the differences to enable better counts.}

{\bf Would be good to conclude this subsection by indicating which approach better if you only have a single source. Let's discuss.}


==> obsolete/experiments.tex <==
This section describes the experimental settings and reports the results.

\subsection{Transfer Scenarios}\label{sec_scenarios}

We conduct a diverse set of experiments to evaluate our proposed methods. We 
%follow three scenarios: 
experiment with three scenarios: 
1) \emph{parallel data}: in this setting, we use both the annotation projection and direct transfer approaches. In order to see the effect of domain and genre, we use different translation datasets: out-of-domain data (religious text), out-of-domain data (contemporary political text) and relatively in-domain data. 
\todo{KM: Below not quite clear. I have tried to rephrase. CHeck if OK.
% In the direct transfer approach, we use the Giza++ \cite{och2000giza} tool to extract the translation dictionaries after getting the intersected alignments from source and target alignment directions. 
 In the direct transfer approach, we produce the intersected alignments from source and target alignment direction and use the Giza++ \cite{och2000giza} tool to extract from these  the translation dictionaries.
We restrict ourselves to the most frequent translation for each word in order to prune alignment noise. 
\todo{KM: is effect of domain and genre measured for both approaches? I think so but if the sentence occurs here, it implies only for direct transfer. I have moved it above. If I am wrong, move back.}
%In order to see the effect of domain and genre, we use different translation datasets: out-of-domain data (religious text), out-of-domain data (contemporary political text) and relatively in-domain data;  
2) \emph{translation dictionaries}: we  use the manual translation dictionaries extracted from Wiktionary\footnote{\url{https://www.wiktionary.org/}} 
\todo{KM: check my rewording}
in place of the dictionaries generated from parallel translations
for the direct transfer model. The Wiktionary entries are noisy and for some languages, the coverage of the lexicon is very restricted; and 3) \emph{comparable corpora}: we use the model of \newcite{??} to extract cross-lingual word embeddings. We use the cross-lingual embeddings as features for the direct transfer method. 
\todo{KM: Check if my rewording OK. I foudn this awkward.}
%This is a minimal setting for the direct transfer method for which we only use the fix pre-trained word embedding features $x_{ce}$.
 We only use the fix pre-trained word embedding features $x_{ce}$ for the direct transfer method in this scenario.


\subsection{Datasets, Tools and Settings}
\todo{KM: wording confusing here. Makes it sound as if only Persian is laveled. I assume not.}
%\paragraph{Labeled sentiment data} We downloaded the tweets for 12 languages 
\paragraph{Labeled sentiment data} We downloaded tweets labeled with sentiment for 12 languages 
from \newcite{tweet_paper} as well as  SentiPers data\footnote{\url{http://dadegan.ir/catalog/sentipers}}, a set of digital products reviews for Persian (fa), as our rich-resource languages. The languages are Bulgarian (bg), German (de), English (en), Spanish (es), Croatian (hr), Hungarian (hu), Polish (pl), Portuguese (pt), Russian (ru), Slovak (sk), Slovene (sl) and Swedish (sv). We split use 80\% of the data as training, 10\% for development and 10\% of the data for testing. We use all development data sets to train the supervised NBSVM models and 
\todo{KM: What is slightly tune? Either drop the word or define.}
slightly tune the parameters for the direct transfer and annotation projection on the Persian development data. 
\todo{KM: I changed the wording below. Check}
%We also use Uyghur, Chinese and Arabic as only the target language. We manually annotated the Uyghur and Chinese data and use the test section of the Arabic Semeval dataset\footnote{\url{http://alt.qcri.org/semeval2017/task4/}}. In the multi-source setting, hold out the training dataset for each language and use other training sets for training. Table~\ref{tab_tweet_size} shows the data sizes.
We also use labeled Uyghur, Chinese and Arabic for the target language only, given smaller amounts of labeled data. We manually annotated the Uyghur and Chinese data and use the test section of the Arabic Semeval dataset\footnote{\url{http://alt.qcri.org/semeval2017/task4/}}. In the multi-source setting, we hold out the training dataset for each language and use the other training sets for training. Table~\ref{tab_tweet_size} shows the data sizes.

\todo{KM: It sounds odd to say here that use U, C and A as ONLY the target language. Why? . To address this I have edited above although we could be called out on that for Arabic. Let's discuss which are low resource languages.}

\input{tweet_data_stat}

\paragraph{Parallel data}
\todo{KM: One problem with the discussion as is, is that you don't describe the domain of the test data. So the out-of-domain descriptions require the reader to think: what is the domain? I think it should be clearly stated above. We can discuss hwere. What exactly is in-domain? Is it product reviews? Or is it any twitter data?}
%As mentioned in \S\ref{sec_scenarios} we use three sets of parallel data. 
We using the following datasets:
\begin{itemize}
    \item \emph{Bible and Quran}: We use the Quran and Bible translations as our out-of-domain  parallel datasets. We use the corpus of \newcite{christodouloupoulos2014massively} for the Bible dataset. This dataset has one translation per language; except for English for which it has two translations. We use both translations of the English data. We use the Tanzil translations\footnote{\url{http://tanzil.net/trans/}} for the holy Quran. This dataset has multiple translations for some languages. 
\todo{KM: CHeck my rewording.}
%We excluded some of the translations from Russian and English because we found them as interpretations and not translations.\footnote{For Russian, we use the Krachkovsky, Kuliev, Osmanov, Porokhova, and Sablukov translations and for English, we use the Ahmedali, Arberry, Daryabadi, Itani, Mubarakpuri, Pickthall, Qarai, Qaribullah, Sahih, Sarwar, Shakir, Wahiduddin, and Yusufali translations.}
We excluded a subset of the  translations from Russian and English that were interpretations as opposed to translations.\footnote{For Russian, we use the Krachkovsky, Kuliev, Osmanov, Porokhova, and Sablukov translations and for English, we use the Ahmedali, Arberry, Daryabadi, Itani, Mubarakpuri, Pickthall, Qarai, Qaribullah, Sahih, Sarwar, Shakir, Wahiduddin, and Yusufali translations.}
    \item \emph{Europarl }: We use the Europarl data \cite{koehn2005europarl} as out-of-domain contemporary political text. We  restricted ourselves to those sentences that are translated to all of the 10 languages (Bulgarian, German, English, Spanish, Hungarian, Polish, Portuguese, Slovak, Slovene, and Swedish). That comprised a total of 294738 sentences for all languages.
    \item \emph{Linguistic Data Consortium (LDC) parallel data}: The LDC consists of in-domain parallel data \todo{KM: Why indomain? State} drawn from Twitter???. We use nine English to target parallel translations from the LDC data: Chinese (16440 sentences)\footnote{LDC2016E30\_LORELEI\_Mandarin}, Persian (57087 sentences)\footnote{LDC2016E93\_LORELEI\_Farsi}, Hungarian (157931 sentences) \footnote{LDC2016E99\_LORELEI\_Hungarian}, Arabic (49446 sentences)\footnote{LDC2016E89\_LORELEI\_Arabic}, Russian (193967 sentences)\footnote{LDC2016E95\_LORELEI\_Russian}, Spanish (345940 sentences)\footnote{LDC2016E97\_LORELEI\_Spanish}, and Uyghur (99272 sentences) \footnote{LDC2016E57\_LORELEI\_IL3\_Incident\_Language\_Pack\_\\for\_Year\_1\_Eval}. 

\end{itemize}


\paragraph{Monolingual text}
We use the Wikipedia dump data set to create monolingual word embeddings and Brown clusters. We also use the monolingual text to train cross-lingual word embeddings and Brown clusters based on the method of \newcite{rasooli_16}: this is done by randomly swapping words in a language with its translation in another language. We replaced X\% of the words in the monolingual corpora with their translations drawn from either the bilingual  dictionary automatically generated from the parallel corpus  or the manual Wiktionary bilingual dictionary.
\todo{KM: Since it is so prominent here, I think we cannot rely on people reading your other paper to understand what is done. It should be defined here. So the last part of this sentence should be made more precise. I've tried but you should edit.}

\paragraph{Pos tagging and tokenization} We use the Universal dependencies corpora \cite{universal_deps} to create training data for sentence and word tokenization, and part-of-speech tagging. We trained sentence tokenization with the OpenNLP toolkit\footnote{\url{https://opennlp.apache.org/}}. We also use the OpenNLP toolkit to train word tokenization for the languages that the Europarl package does not provide a tokenization script; except Arabic, Persian and Chinese. For Chinese we use the Stanford Chinese segmenter \cite{chinese_segmentor}, Madamira \cite{pasha2014madamira} with ATB tokenization format for Arabic, and the Hazm toolkit\footnote{\url{https://github.com/sobhe/hazm}} for Persian.  We trained the perceptron-based part-of-speech tagger of \newcite{collins2002discriminative}\footnote{\url{https://github.com/rasoolims/SemiSupervisedPosTagger}} for training our tagging models.
\todo{KM: A question will come up here: you needed data labeled with POS for each language, correct? Did you have it?}

\paragraph{Comparable data}\todo{MSR: Noura; please fill this in. If you want to add any table for statistics; please put in in another tex file and use \\input\{\} for that}

\paragraph{Embeddings and Brown clusters} We use the Word2vec tool\footnote{\url{https://code.google.com/archive/p/word2vec/}} with its default setting and dimension of 300 for all of our embeddings (monolingual and cross-lingual). We trained monolingual and cross-lingual Brown clusters with the method of \newcite{stratos2014spectral}\footnote{\url{https://github.com/karlstratos/singular}} with 500 clusters.

\paragraph{Neural network model} We have implemented our neural network model by using the Dynet library \cite{neubig2017dynet}. We use seven iterations for the single-source transfer experiments and two epochs for the multi-source transfer (concatenation of multiple sources). We use the following dimensions for all of our experiments: pre-trained word embeddings $d_{ce}=300$, updatable word embeddings $d_{e}=400$, cross-lingual Brown cluster embeddings $d_{cc}=50$, batch size of 10K, LSTM output dimension $d_{rec}=400$, and hidden layer dimension $d_h = 400$.


\subsection{Baseline approach}
We provide a simple baseline to compare all of our methods: this is done by translating the Sentiwordnet \cite{baccianella2010sentiwordnet} lexicon to each target language by using the dictionaries extracted from the Bible and Quran parallel data. We use a simple threshold to determine the sentiment assignment for each sentence:

\[
l(x)=
\begin{cases}
\text{positive} & s_x[p]-s_x[n]>\delta \\
\text{negative} & s_x[n]-s_x[p]>\delta \\
\text{neutral} & \text{otherwise} \\
\end{cases}
\]

$s_x[p]$ and $s_x[n]$ show the average positive and negative  sentiwordnet score for the words in a sentence $x$. We chose $\delta = 0.1$ based on the performance on the Persian development data.

\subsection{English to Target Transfer Results}
In our first set of experiments, we conduct the transfer experiments by transferring only from the English language. In cases where we have more than one translation for a sentence (such as Quran), we apply majority voting to get the most frequent label. The results are depicted in Table~\ref{tab_single_results}. \todo{MSR: after having all numbers,  I will write more. the results for the projection will be updated; some numbers are wrong. Will update it asap}

\input{single_table}

\subsection{Multi-Source Transfer Results}
In this set of experiments, we use all training data sets (except the one for the target language) as the source language in the experiments. For annotation projection, we apply majority voting on sentences with more than one translation. For direct transfer we apply three different techniques: 1) Concatenation: we concatenate all the training sets and use it as the training data; 2) Ensemble-flat: for every source language, we train a single-source direct transfer method and run the trained model on the testing data. We then use the most frequent label assignment on the testing data; 3) Ensemble-KL: this is very similar to the Ensemble-flat method, except that we weigh every label assignment proportional to the KL-divergence of the target and source POS trigram distribution. We use the method of \newcite{rosa-zabokrtsky:2015:ACL-IJCNLP} in which we use the fourth power of the inverted value the KL-divergence.\footnote{We also tried the cosine similarity but similar to \cite{rosa-zabokrtsky:2015:ACL-IJCNLP} we did not see any improvement.}
\todo{KM: THink about whether we should include both ensemble-flat and ensemble-KL.}

Table~\ref{tab_multi_source_results} shows the results for different settings.\todo{the results for the projection will be updated; some numbers are wrong. Will update it asap}

\input{multi_source_table}


==> obsolete/intro.tex <==

%There has been a great deal of interest in sentiment analysis \cite{liu2012sentiment,rosenthal2014semeval,rosenthal2015semeval,nakov2016semeval}. 
%\todo{KM: intro needs to be reworked. Needs better motivation for why sentiment and why low resource. I can do on weekend.}\todo{MSR: I am not very familiar with the applications of SA. So I thought to write something naiive for motivation and then you or Noura will change it. Thanks}
Online discussion forums and social media are often used to express subjective views. 
Social media is  frequently exploited  to express  political viewpoints or to post reviews, but it can also be used in  serious situations such as disasters where people post about their experiences. In such cases, negative sentiment can be an indication of continued problems while positive sentiment can be an indication that the situation has been happily resolved. 
Sentiment analysis involves predicting the polarity of a given sentence or phrase  as negative or neutral.  While there has been quite bit of work on recognition of sentiment in English  (e.g.,~\cite{ Cardie, Wiebe, some more recent ones}), there is only beginning to be research  in languages such as Chinese~\cite{?}, Arabic~\cite{?} and  Spanish~\cite{?}) and there has been very little work in many low resource languages where datasets labeled for sentiment do not exist. Yet situations requiring humanitarian assistance can  occur in areas where low resource languages are spoken; for example,  the remote mountainous region of X where Uyghur is spoken was the site of a major earthquake while under-developed areas such as Y where Z is spoken may require assistance in case of drought or disease outbreaks.
 Recognizing the sentiment of online content can help humanitarian organizations identify the areas of greatest need. 

 Our goal is to create robust sentiment analysis systems for languages for which no labeled training data is available. To obtain this objective, we experiment with  different transfer techniques to transfer sentiment information from one or more resource-rich languages to a low resource target language.

\todo{I don't think we should refer to transfer for sentiment right up front. SHould we? Might be better to compare in more detail in related work. I commented out.}
Methods for transferring linguistic information have been used in several tasks such as
% sentiment analysis (e.g. \newcite{chen2016adversarial} 
% \newcite{zhou-wan-xiao:2016:EMNLP2016}), 
part-of-speech tagging (e.g. \newcite{tackstrom2013token}), dependency parsing (e.g. \newcite{mcdonald-petrov-hall:2011:EMNLP}) and semantic role labeling (e.g. \newcite{akbik-EtAl:2015:ACL-IJCNLP}). 
%KM - This is repetitive. 
%The goal of transfer methods is to transfer information and/or annotation from a set of rich-resource languages to a target language. 
Different techniques such as annotation projection through translation data (e.g. \newcite{mihalcea-banea-wiebe:2007:ACLMain}), direct transfer of a supervised model (e.g. \newcite{Zhou2014}), and machine translation (e.g \cite{wan:2008:EMNLP1,Wan:2009:CCS:1687878.1687913,Duh:2011:MTR:2002736.2002823,balahur2014comparative,zhou-wan-xiao:2016:P16-1,zhou-wan-xiao:2016:EMNLP2016}) have been used to transfer linguistic information accross languages. 

Previous work \cite{mihalcea-banea-wiebe:2007:ACLMain,wan:2008:EMNLP1,Wan:2009:CCS:1687878.1687913,Duh:2011:MTR:2002736.2002823,balahur2014comparative,zhou-wan-xiao:2016:P16-1,zhou-wan-xiao:2016:EMNLP2016} mostly assume the availability of rich resources such as a machine translation system or a huge parallel corpus. Unfortunately this is not the situation in many low-resource languages. 
Furthermore, previous work has focused on a small number of languages and has solely used English as the source language.  

In this paper, we show that we can have an accurate system in the absence of rich resources. 
We consider a cross-lingual scenario in which multiple source languages are used to transfer information to a target language. 
We consider two main approaches for transfer:  \emph{annotation projection} and \emph{direct transfer}. For the projection approach, we use translation data to project supervised labels from the source languages to the target language. When we have multiple source translations, we apply majority voting to yield  more robust projected data. For the direct transfer approach, we directly train a sentiment analysis system on the  labeled sentences of the source language(s)  and apply the trained model directly on the target language. We show that by using a small cross-lingual dictionary, we can adapt the input features to generalize well to the target language. 
\todo{KM: What does ``flexible enough'' mean? Do you mean ``can be flexibly applied to different data scenarios'' or do you mean that you can achieve good results with it? I think we have to think carefully how to present results so I would not include the second. I changed to mean the first. }
\S\ref{sec_approach} gives more details about the two approaches. We show that the direct transfer method is flexible and can be applied to different data availability scenarios (parallel data, comparable corpora, and manual dictionaries).

The main contributions of this paper are:
%\todo{KM: I think the use of code-switched data should be mentioned. I also would be in favor of previewing results of experiments if we can figure that out. Perhaps that for some languages projection better and for others transfer, but that if voting transfer from multiple source languages is used, on average we see bet result. Tao- saw your email and you should experiment with the dictionaries.}\todo{MSR: On average and also one most of the languages direct does better but it is a tough question to answer if it is because of the neural network vs SVM or something else. I think it is not possible to use dictionaries with projections.}
\begin{itemize}
    \item We introduce a novel direct transfer method. It is a deep neural netwrok model based on recurrent neural networks \cite{medsker2001recurrent} and multilayer perceptron. We use a simple but effective approach to translate the words in monolingual corpora, and also make use of cross-lingual word representations. 
\todo{KM: Does the last half of the sentence above fit?}
The translated input sentences  resemble code-switched text where some of the words belong to the source language and some others belong to the target language. Therefore, our model does not rely on having fully translated text.
    \item We introduce a simple but effective annotation projection strategy. We show that by using multiple source languages, we can alleviate the projection noise.
    \item We systematically experiment with different methods based on direct transfer and projection to develop sentiment analysis systems in the absence of rich resources. Our experiments on a set of different languages show that we can create a very robust model. Our experiments show 
 the effect of having in-domain vs. out-of-domain translation data, single-source vs. multi-source transfer,  manual dictionaries vs. parallel data, and comparable corpora in the absence of any parallel translated data.
\end{itemize}


Experiments show ....






==> obsolete/multi_source_table.tex <==
\begin{table*}[t!]
    \centering
    \begin{tabular}{c|c | c c | c | c  c c  c | c c c c | c}
    \hline \hline
       \multirow{3}{*}{L.} & \multirow{3}{*}{${\cal B}$}   & \multicolumn{2}{c|}{{\bf Projection}}  & \multirow{3}{*}{Sup.}   & \multicolumn{8}{c|}{{\bf Direct}} & \multirow{3}{*}{Sup.}   \\ 
        & & \multirow{2}{*}{BQ} & \multirow{2}{*}{EP} & & \multicolumn{4}{c|}{BQ} & \multicolumn{4}{c|}{EP} & \\
        & & & & & SB ($L_{s^*}$)  & EF & EK & CT & SB ($L_{s^*}$) & EF & EK & CT & \\ \hline
ar & 39.3 & 46.1 & -- & -- & 42.4 (sk) & 42.4 & 43.6 & 39.9 & -- & -- & -- & -- & --\\ 
bg & 46.9 & 48.9 & 43.7 & 60.5 & 52.6 (hu) & 50.9 & 46.6 & 43.7 & 54.9 (en) & 51.3 & 48.4 & 49.3 & 60.0\\ 
de & 53.5 & 57.1 & 43.9 & 63.2 & 58.1 (en) & 57 & 59.2 & 56.5 & 60.4 (en) & 57.7 & 60.4 & 51.8 & 66.2\\ 
en & 50.4 & 53 & 43.5 & 65.1 & 52.7 (sv) & 55.2 & 56 & 53.3 & 53.9 (de) & 55 & 55.5 & 55.7 & 66.0\\ 
es & 41.1 & 41.4 & 43.1 & 59 & 48.7 (fa) & 48.7 & 47.8 & 47.7 & 48.7 (es) & 49.3 & 46.4 & 46.9\\ 
fa & 38.6 & 40.1 & -- & 83.9 & 52.4 (es) & 45.2 & 43.2 & 53.9 & -- & -- & -- & --\\ 
hr & 26.8 & 44.0 & -- & 66.4 & 52.1 (hu) & 45.5 & 42.8 & 43.4 & -- & -- & -- & -- & 67.9\\ 
hu & 36.0 & 33.7 & 49.7 & 65.3 & 54.8 (ru) & 53.8 & 51.8 & 55.2 & 51.9 (pl) & 51.1 & 49.0 & 56.1 & 67.1\\ 
pl & 30.3 & 41.8 & 51.4 & 66.3 & 46.3 (hu) & 50.4 & 46.6 & 42.1 & 50.8 (hu) & 48.7 & 53.2 & 56\\ 
pt & 34.6 & 38.6 & 36.1 & 51.4 & 39.6 (hr) & 39.1 & 36.9 & 36.2 & 40.9 (en) & 39.4 & 38.1 & 38.3\\ 
ru & 41.2 & 45.7 & -- & 68.0 & 47.7 (en) & 45.4 & 44.8 & 48.2 & -- & -- & -- & --\\ 
sk & 25.0 & 40.2 & 45.6 & 70.2 & 50.0 (pl) & 35.0 & 38.9 & 48.7 & 53.2 (pl) & 45.3 & 49.0 & 50.4 & 72.2\\ 
sl & 44.6 & 41.0 & 44.9 & 59.0 & 48.2 (hr) & 45.5 & 44.1 & 43.6 & 48.2 (bg) & 47.9 & 49.0 & 46.3 & 58.4\\ 
sv & 33.5 & 45.6 & 47.9 & 64.0 & 49.3 (de) & 44 & 45.2 & 45.3 & 50.4 (en) & 49.7 & 50.2 & 47.3\\ 
ug & 46.8 & 57.0 & -- & -- & 54.9 (fa) & 48.6 & 54.9 & 35.3 & -- & -- & -- & -- & --\\ 
zh & 45.6 & 52.2 & -- & -- & 48.9 (fa) & 48.0 & 47.0 & 32.0 & -- & -- & -- & -- & --\\    \hline
avg & 39.6 & 45.4 & 45.0 & 63.9 & & 47.2 & 46.8 & 45.3 & & 49.5 & 49.9 & 49.8 & 65.4\\  \hline \hline

    \end{tabular}
    \caption{Accuracies for different setting in multi-source experiments. ${\cal B}$ shows the baseline results using translated Sentiwordnet. The two annotation projection results using the Bible and Quran (BQ) and Europarl data (EP) and the supervised accuracy of the NBSVM model are shown in columns 3-5. The different settings in the direct model are shown in the right major columns. ``SB'' shows the best source language for each target, ``EF'' is the ensemble-flat and ``EK'' is the ensemble-kl divergence, and ``CT'' is the direct model trained on the concatenated training data sets.}
    \label{tab_multi_source_results}
\end{table*}

==> obsolete/neural_fig.tex <==
\begin{figure*}[!th]
    \centering
    
    \includegraphics[width=0.95\textwidth]{senti_lstm}
    \caption{A graphical depiction of the neural network model in our direct transfer approach. This is an example of an English tweet translated to German. The words are shown at the bottom with their translation appearing after colon (``:''). The first and the last words are emojies. The circles ($f_i$) show the embedding layer, the LSTMs are shown on top of the embedding layer and the average pool layer on the right side of the words. All the intermediate layers are concatenated and fed to a multi-layer perceptron  (MLP). More details are given in \S\protect\ref{sec_direct}.}
    \label{fig_neural_fig}
\end{figure*}

==> obsolete/obsolete.tex <==
%We agree that data privacy is important in many cases. However, privacy does not matter when we are querying public or internal datasets. It is better for the system be able to interact with users, search users' requests in the database, and show results and double check with users to finalize answers. \textcolor{red}{How about removing this paragraph?}

%Our contributions in this paper are two-fold. First, we propose a type attention mechanism to solve the problem of rare words and numbers commonly faced by the language-to-SQL parser. We group words in the entities found in knowledge graph, and numbers and column names in the questions. Moreover, our model significantly improves training stability and accuracy. It also increases the training speed more than three times compared with all previous models (converge to a higher accuracy in much fewer epochs). On a side note, our training procedure does not require multiple steps as previous works did.

%Second, we study the performances of the parser under different settings. Specifically, we evaluate our model under two main settings, content-free and content-sensitive. We show that content aware system could answer some incomplete queries correctly by looking into the database. Therefore, we can have a more robust and accurate language-to-SQL parser with access to the database.

\iffalse
Before we proceed, we define two core procedures of our model:
\begin{itemize}
    \item \textbf{ATTENTION} procedure averages a matrix $\newvec{H}_2$ based on another matrix $\newvec{H}_1$ via an intermediate \emph{attention score} $\alpha$.
    \begin{gather*}
    \alpha = \softmax(\newvec{H}_1^\top \newvec{W} \newvec{H}_2) \\
    \textbf{ATTENTION}(\newvec{H}_1,\newvec{H}_2) = \alpha \newvec{H}_2
    \end{gather*}
    where $\newvec{W}$ is a learnable matrix.
    \item \textbf{PREDICTION} procedure generates a probability distribution given matrices $\newvec{H}_1,\dots,\newvec{H}_n$.
    \begin{gather*}
    \beta = \newvec{U} \tanh (\sum_{i=1}^n \newvec{W}_i\newvec{H}_i) \\
    \textbf{PREDICTION}(\newvec{H}_1,\dots,\newvec{H}_n)= \softmax(\beta)
    \end{gather*}
     where \{$U$,$W_1,\dots,W_n$\} are learnable matrices.
\end{itemize}
Unless specified otherwise, all procedures do not share parameters.
\fi

\iffalse
$$H_{qt/col} = \textbf{ATTENTION}(H_{col},H_{qt})$$
\fi

\iffalse
$$P_{sel}(col/qt)= \textbf{PREDICTION}(H_{col},H_{qt/col})$$
\fi

\iffalse
\begin{multline*}
P_{num}(k/qt, col) =  \textbf{PREDICTION}(H_{qt/col_1}, \\
H_{qt/col_2},H_{qt/col_3},H_{qt/col_4})
\end{multline*}
\fi

\iffalse
$$H_{qt/agg} = \textbf{ATTENTION}({H_{agg}, H_{qt}})$$
\fi

\iffalse
$$P_{agg}(agg/qt, col)= \textbf{PREDICTION}(H_{ct},H_{qt/agg})$$
\fi

\iffalse
$$P_{op}(op/qt, col) = \textbf{PREDICTION}(H_{ct},H_{qt/colt})$$
\fi

\iffalse
$$P_{val}(w_i/qt, col, h) = \textbf{PREDICTION}(H_{ct},H_{qt/col}, h)$$
\fi

\iffalse
\subsection{Models}
\textbf{SQL+Q: } Model only uses questions as its input.

\textbf{SQL+QC: } Model only uses question and column names as inputs.

\textbf{SQLKG+QC: } Our main model comparable to previous works on WikiSQL dataset. It uses questions, column names and type attention but no content of databases as inputs.

\textbf{SQLKG+TC: } model uses question, column names, type attention by fully access to content of databases.
\fi

Semantic parsing maps natural language to meaningful executable programs. The programs could be a range of representations such as logic form \cite{zelle96,Zettlemoyer05,wong07,Das10,Liang11,banarescu13,artzi13,Reddy14,Berant14,pasupat2015compositional,Yin15}.
The main focus of our paper is on translating natural language into SQL queries. \cite{Poon13}
\cite{li2014constructing}

==> obsolete/related.tex <==
There has been a great deal of interest in transfer methods for sentiment analysis. In summary, the main difference of this paper to previous work is on the limited data availability assumptions in this paper compared to the need for machine translation systems in previous work. Furthermore, to the best of our knowledge, ours is the first work that conducts a diverse set of experiments with multiple source languages, with and without parallel data, using the annotation projection and direct transfer approaches. 

Unlike other natural language processing tasks such as parsing in which the direct transfer and annotation projection methods are the mostly used techniques, most of the methods in sentiment analysis transfer use the \emph{machine translation} approach \cite{wan:2008:EMNLP1,Wan:2009:CCS:1687878.1687913,Duh:2011:MTR:2002736.2002823,balahur2014comparative,zhou-wan-xiao:2016:P16-1,zhou-wan-xiao:2016:EMNLP2016}. This approach uses a standard machine translation system to translate the gold-standard source (usually English) data to a target language and then train a sentiment analysis system on the target language. There are extensions to the basic translation approach: e.g., \newcite{zhou-EtAl:2015:ACL-IJCNLP2} tries to correlate the word and document representations of the source and target languages based on sentiment polarity and translation indicators. \newcite{zhou-wan-xiao:2016:EMNLP2016} develops an attention model to learn a sentiment analysis system after running machine translation on the source labeled data. 


Our direct transfer approach is slightly similar to the machine translation approach with the following differences: first, we do not need to fully translate the source languages text, and even if we only have cross-lingual word representations (embeddings and clusters), it is not essential to have a cross-lingual dictionary. Moreover, our method does not apply any reordering or structural changes to the source sentences. It is worth noting that there are some few papers that use direct transfer without using machine translation: e.g., \newcite{Zhou2014} design a neural network model by projecting the embeddings of the source and target languages into a shared space using parallel data. They only apply their method on the English to Chinese sentiment transfer task. 



%\newcite{chen2016adversarial}  create shared representation by introducing multi-task learning in which the second task is the prediction of language.
\newcite{mihalcea-banea-wiebe:2007:ACLMain} apply an annotation projection method using a single-source setting with English as the source language. \newcite{li2016structural} map the feature space of a source language to a target language the structural correspondence learning (SCL). This is very similar to learning cross-lingual word representations in the sense that those representations are the actual features for the sentiment analysis system.  \newcite{meng-EtAl:2012:ACL2012} increases the coverage of sentiment lexicons for a resource-poor language by using automatic word alignments on parallel data.  

The use of comparable corpora is under-studied in previous work. \newcite{zagibalov2010comparable} studied the use of comparable corpora for the Russian and English languages. \newcite{martinezcamara-EtAl:2013:WASSA} make use comparable corpora for opinion mining.

There has been a great deal of work on inducing cross-lingual word representations (e.g. see \newcite{tackstrom2012cross}, \newcite{hermann2013multilingual}, \newcite{faruqui-dyer:2014:EACL},  \newcite{ammar2016massively}). In this paper, we use the simple method of \newcite{rasooli_16} that is based on applying artificial code-switching on monolingual text by using cross-lingual dictionaries. This method is very similar to the method of \newcite{gouws-sogaard:2015:NAACL-HLT} and \newcite{wick-et-al-2016}.

==> obsolete/single_table.tex <==
\begin{table*}[ht!]
    \centering
    \small
    %\setlength{\tabcolsep}{2pt}
    \begin{tabular}{c|c | c c c c | c c c c c c }
    \hline \hline
    \multirow{2}{*}{L.} & \multirow{2}{*}{${\cal B}$}   & \multicolumn{3}{c}{Projection}  & \multirow{2}{*}{Sup.}   & \multicolumn{5}{c}{Direct} & \multirow{2}{*}{Sup.}   \\ 
         &  & $BQ$ & $EP$ & $LDC$ & & $CP$ & $WK$ & $BQ$ & $EP$ & $LDC$ &  \\ \hline
ar & 39.3 & 40.6 & -- & 44.9 & -- & & 37.7 & 41.1 & -- & 41.8 & --\\ 
bg & 46.9 & 51.5 & 52.5 & -- & 60.5 & & 49.9 & 52 & 54.9 & -- &\\ 
de & 53.5 & 58.1 & 58.3 & -- & 63.2 & & 57.3 & 58.1 & 60.4 & -- &\\ 
es & 41.1 & 46.7 & 46.9 & 47.6 & 59.0 & & 46.3 & 46.5 & 43.8 & 49.1& \\ 
fa & 38.6 & 40.4 & -- & 42.0 & 83.9 & & 37.6 & 51.2 & -- & 39.3 &\\ 
hr & 26.8 & 30.0 & -- & -- & 66.4 & & -- & 39.7 & -- & -- & \\ 
hu & 36.0 & 42.4 & 42.4 & 50.5 & 65.3 & & 44.6 & 42.4 & 37.7 & 45.2 &\\ 
pl & 30.3 & 39.8 & 39.8 & -- & 66.3 & & 38.8 & 43 & 46 & -- &\\ 
pt & 34.6 & 39.7 & 39.7 & -- & 51.4 & & 40.3 & 39.5 & 40.9 & -- &\\ 
ru & 41.2 & 45.0 & -- & 49.3 & 68.0 & & 50.2 & 47.7 & -- & 53.8 &\\ 
sk & 25.0 & 31.7 & 31.7 & -- & 70.2 & & 49.4 & 26.9 & 27.3 & -- &\\ 
sl & 44.6 & 50.2 & 50.2 & -- & 59.0 & & 40.7 & 44.5 & 47.8 & -- &\\ 
sv & 33.5 & 46.0 & 46.0 & -- & 64.0 & & 43.9 & 40.4 & 50.4 & -- & \\ 
ug & 46.8 & 54.0 & -- & 46.8 & -- & & 30.9 & 37.9 & -- & 46.2 & -- \\ 
zh & 45.6 & 51.2 & -- & 59.1 & -- & &  69.2 & 46.6 & -- & 58.1 & --  \\ \hline
avg & 39.6 & 44.5 & 45.3 & 48.6 & 64.7 & & 45.5 & 43.8 & 45.5 & 47.6 & \\ \hline \hline

    \end{tabular}
    
    \caption{Accuracies of different methods in the single-source (English to target) transfer setting. ``${\cal B}$'' refers to the baseline method. The two ``sup.'' columns refer to the supervised NBSVM and neural network models (an upper-bound for the projection and direct transfer methods respectively). ``CP'' refers to the use of embeddings extracted from comparable corpora, ``WK'' refers to the full direct model using the Wiktionary lexicon. ``BQ'', ``EP'' and ``LDC'' refer to the different parallel datasets used in our experiments: Bible and Quran as ``BP'', Europarl as ``EP'' and the LDC in-domain translation datasets.}
    \label{tab_single_results}
\end{table*}

==> obsolete/tweet_data_stat.tex <==
\begin{table}[!th]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{4.5pt}
    \begin{tabular}{c|c c c | c c c}
    \hline \hline
         \multirow{2}{*}{Dataset}   & \multicolumn{3}{c|}{Train}  &  \multicolumn{2}{c}{Test} \\  \cline{2-7} 
          & \#sen & \#tok & \#types & \#sen & \#tok & \#types \\ \hline
ar & -- & -- & -- & 6100 & 115401 & 19474 \\ 
bg & 23739 & 313003 & 52922 & 2958 & 38685 & 12545 \\ 
de & 63669 & 822605 & 78353 & 7961 & 102822 & 19907 \\ 
en & 46623 & 601284 & 39294 & 5828 & 75147 & 10857 \\ 
es & 137106 & 2007046 & 91419 & 17133 & 249690 & 27942 \\ 
fa & 15000 & 331431 & 13840 & 3027 & 67926 & 6886 \\ 
hr & 56212 & 726037 & 88966 & 7025 & 90544 & 23827 \\ 
hu & 36167 & 427951 & 83931 & 4520 & 53588 & 17750 \\ 
pl & 116105 & 1455273 & 136089 & 14517 & 182194 & 37018 \\ 
pt & 62989 & 712852 & 41982 & 7872 & 89553 & 12440 \\ 
ru & 44757 & 522218 & 84463 & 5594 & 64779 & 18823 \\ 
sk & 40470 & 576611 & 82281 & 5058 & 71131 & 20751 \\ 
sl & 74238 & 1106211 & 108735 & 9277 & 137371 & 29899 \\ 
sv & 32600 & 494139 & 42446 & 4074 & 61423 & 11698 \\ 
ug & -- & -- & -- & 346 & 6805 & 3560 \\ 
zh & -- & -- & -- & 487 & 10243 & 3213 \\  \hline \hline
    \end{tabular}
    \caption{Training and evaluayion sizes for different languages in our experiments. We ignored the hash tags (tokens starting with \#), urls and name mentions (tokens starting with @) in the data.}
    \label{tab_tweet_size}
\end{table}

==> results_table_cp.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.92}{
\begin{tabular}{cccccc}
\hline
 Method                         & Easy    & Medium  & Hard   & Extra Hard & All    \\ \hline
                                \multicolumn{6}{c}{Example Split} \\ \hline
Seq2Seq                         & 24.3\%	& 9.5\%	& 6.3\%	& 1.5\%	& 11.2\% \\
Seq2Seq+Attention \cite{dong16} & 31.2\%  & 13.9\%   & 11.6\%  & 3.3\%      & 15.5\%  \\
Seq2Seq+Copying                 & 30.0\%	& 12.6\%	& 10.0\%   & 3.3\% & 14.8\% \\
%Seq2Seq                          & 38.5\%  &  20.1\%  &  14.4\%  &  8.2\%   &  21.6\% \\
%Seq2Seq+Attention \cite{dong16}  & 57.3\%  &  39.0\%  &  32.8\%  &  20.7\%  &  39.4\% \\
%Seq2Seq+Copying                  & 51.4\%  &  33.3\%  &  24.7\%  &  15.8\%  &  33.3\% \\
\newcite{iyer17}                & 18.6\%  & 12.0\%   & 9.0\%   & 1.8\%      & 9.8\%  \\
% Seq2SQL \cite{Zhong2017}        & 4.3\%   & 2.7\%    & 0.0\%   & 0.0\%      & 2.2\%  \\
SQLNet \cite{Xu2017}            & 36.2\%  & 15.6\%   & 7.9\%   & 4.9\%      & 17.4\%  \\
TypeSQL \cite{Yu18}             & 48.6\%  & 38.2\%   & 18.1\%  & 19.8\%     & 34.3\%  \\ \hline
                                \multicolumn{6}{c}{Database Split} \\ \hline
Seq2Seq                         & 17.9\% & 2.7\% & 1.3\% & 0.6\% & 5.4\% \\
Seq2Seq+Attention \cite{dong16} & 17.9\%  & 2.9\%   & 1.8\%  & 1.3\%      & 5.7\%  \\
Seq2Seq+Copying                 & 15.1\%  & 3.4\%	& 1.0\%	& 1.3\%	& 5.2\% \\
%Seq2Seq                          & 17.7\%  &  3.9\%  &  3.5\%  &  0.6\%  &  6.4\% \\
%Seq2Seq+Attention \cite{dong16}  & 20.3\%  &  5.5\%  &  5.5\%  &  1.6\%  &  8.2\% \\
%Seq2Seq+Copying                  & 20.9\%  &  5.5\%  &  6.5\%  &  1.6\%  &  8.5\% \\
\newcite{iyer17}                & 7.9\%   & 2.1\%   & 1.3\%  & 1.1\%      & 3.1\%  \\
% Seq2SQL \cite{Zhong2017}        & 1.9\%   & 0.5\%   & 0.0\%  & 0.0\%      & 0.7\%  \\
SQLNet \cite{Xu2017}            & 23.7\%  & 5.9\%   & 2.3\%  & 0.3\%      & 8.3\%  \\
TypeSQL \cite{Yu18}             & 29.6\%  & 6.1\%   & 2.3\%  & 0.3\%      & 9.7\%  \\ \hline   
\end{tabular}}
\vspace{-2mm}
\caption{Accuracy of Exact Matching on SQL queries with different hardness levels.}
\label{tab:results}
\vspace{-1mm}
\end{table*}

\begin{table*}[ht!]
\centering
\scalebox{0.92}{
\begin{tabular}{ccccccc}
\hline
 Method           & \texttt{SELECT} & \texttt{WHERE} & \texttt{GROUP BY} & \texttt{ORDER BY} & \texttt{KEYWORDS} \\\hline
                  \multicolumn{6}{c}{Example Split} \\ \hline
Seq2Seq           & 25.8\% & 8.2\% & 18.9\% & 13.0\%  & 21.8\% \\
Seq2Seq+Attention & 30.0\% & 11.4\% & 24.1\% & 19.3\% & 22.4\% \\
Seq2Seq+Copying   & 28.7\% & 8.7\% & 24.2\% & 21.6\% & 19.7\% \\
%Seq2Seq           & 53.0\%  &  33.2\%  &  27.5\%  &  37.1\%  &  56.2\% \\
%Seq2Seq+Attention & 68.4\%  &  57.4\%  &  49.5\%  &  59.0\%  &  69.7\% \\
%Seq2Seq+Copying   & 60.1\%  &  50.6\%  &  42.1\%  &  55.1\%  &  59.6\% \\
\newcite{iyer17}  & 19.2\% & 8.1\% & 16.1\% & 9.6\% & 13.6\% \\
%Seq2SQL           & 0.147 & 1 & 0.085 & 0.096 & 1 & 0.179 \\
SQLNet            & 46.1\% & 32.5\% & 30.6\% & 61.4\% & 77.6\% \\
TypeSQL           & 68.7\% & 55.4\% & 40.5\% & 67.0\% & 73.6\% \\ \hline
                  \multicolumn{6}{c}{Database Split} \\ \hline
Seq2Seq           & 13.7\% & 3.7\%  & 3.2\% & 4.9\% & 8.9\% \\
Seq2Seq+Attention & 14.0\%	& 5.0\%	& 3.2\%	& 6.1\%	& 9.4\% \\
Seq2Seq+Copying   & 12.0\%	& 2.7\%	& 5.2\%	& 6.9\%	& 6.7\% \\
%Seq2Seq           & 21.9\%  &  8.2\%  &  6.3\%  &  15.5\%  &  23.2\% \\
%Seq2Seq+Attention & 23.6\%  &  12.1\%  &  7.0\%  &  19.4\%  &  25.5\% \\
%Seq2Seq+Copying   & 21.8\%  &  14.0\%  &  10.1\%  &  18.0\%  &  20.7\% \\
\newcite{iyer17}  & 6.3\%	& 1.9\%	& 3.0\%	& 3.6\%	& 3.5\% \\
%Seq2SQL           & 0.052	& 1	    & 0.035	& 0.07	& 1	    & 0.219 \\
SQLNet            & 24.0\%	& 18.0\%  & 11.8\% &  47.1\%	& 61.9\% \\
TypeSQL           & 36.2\%	& 14.7\%  & 6.4\%	& 49.5\%	& 59.4\% \\ \hline
\end{tabular}}
\vspace{-2mm}
\caption{F1 scores of Component Matching on all SQL queries.}
\label{tab:results_component}
\vspace{-3mm}
\end{table*}

==> results_table_cp2.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.92}{
\begin{tabular}{c|ccccc|c}
\hline
                                & \multicolumn{5}{c|}{Test} & Dev \\
                          & Easy    & Medium  & Hard   & Extra Hard & All & All   \\ \hline
                                \multicolumn{6}{c}{Example Split} \\ \hline
Seq2Seq                         & 23.6 & 7.9 & 5.5 & 1.3 & 9.8 & 10.7  \\
Seq2Seq+Attention \cite{dong16} & 33.3 & 15.8 & 10.3 & 2.3 & 16.2 & 16.5   \\
Seq2Seq+Copying                 & 30.3 & 13.2 & 8.8 & 3.0 & 14.4 & 15.4  \\
SQLNet \cite{Xu2017}            & 45.9 & 20.5 & 12.4 & 3.3 & 21.5 & 22.0   \\
TypeSQL \cite{Yu18}             & 57.2 & 39.4 & 24.1 & 14.4 & 35.6 & 37.5   \\ \hline
                                \multicolumn{6}{c}{Database Split} \\ \hline
Seq2Seq                         & 17.3 & 1.9 & 1.3 & 0.5 & 4.9 & 3.8  \\
Seq2Seq+Attention \cite{dong16} & 18.1 & 2.6 & 2.0 & 1.1 & 5.6 & 2.7   \\
Seq2Seq+Copying                 & 15.8 & 3.4 & 2.0 & 1.1 & 5.4 & 4.1  \\
SQLNet \cite{Xu2017}            & 35.6 & 13.3 & 6.6 & 1.3 & 14.7 & 14.3   \\
TypeSQL \cite{Yu18}             & 29.9 & 7.6 & 4.0 & 0.8 & 10.5 & 10.6   \\ \hline   
\end{tabular}}
\vspace{-2mm}
\caption{Accuracy of Exact Matching on SQL queries with different hardness levels.}
\label{tab:results}
\vspace{-1mm}
\end{table*}

\begin{table*}[ht!]
\centering
\scalebox{0.92}{
\begin{tabular}{ccccccc}
\hline
 Method           & \texttt{SELECT} & \texttt{WHERE} & \texttt{GROUP BY} & \texttt{ORDER BY} & \texttt{KEYWORDS} \\\hline
                  \multicolumn{6}{c}{Example Split} \\ \hline
Seq2Seq           & 23.3 & 4.9 & 15.3 & 9.2 & 17.9  \\
Seq2Seq+Attention & 31.1 & 9.1 & 28.2 & 20.8 & 21.4  \\
Seq2Seq+Copying   & 28.2 & 8.3 & 25.5 & 21.3 & 19.0  \\
SQLNet            & 59.8 & 32.9 & 35.9 & 65.5 & 76.1  \\
TypeSQL           & 77.3 & 52.4 & 47.0 & 67.5 & 78.4  \\ \hline
                  \multicolumn{6}{c}{Database Split} \\ \hline
Seq2Seq           & 13.0 & 1.5 & 3.3 & 5.3 & 8.7  \\
Seq2Seq+Attention & 13.6 & 3.1 & 3.6 & 9.9 & 9.9  \\
Seq2Seq+Copying   & 12.0 & 3.1 & 5.3 & 5.8 & 7.3  \\
SQLNet            & 44.5 & 19.8 & 29.5 & 48.8 & 64.0 \\
TypeSQL           & 36.4 & 16.0 & 17.2 & 47.7 & 66.2 \\ \hline
\end{tabular}}
\vspace{-2mm}
\caption{F1 scores of Component Matching on all SQL queries on Test set.}
\label{tab:results_component}
\vspace{-3mm}
\end{table*}
